UniTS: Unified Spatio-Temporal Generative Model for Remote Sensing

One of the primary objectives of satellite remote sensing is to capture the complex dynamics of the Earth environment, which encompasses tasks such as reconstructing continuous cloud-free image sequences, detecting land cover changes, and forecasting future surface evolution. However, existing methods typically require specialized models tailored to different tasks, and lack a general framework that can address these multi-level tasks from a unified perspective. In this paper, we propose a Unified Spatio-Temporal Generative Model (UniTS), which integrates several long-separated core tasks, including time series reconstruction, time series cloud removal, time series semantic change detection, and time series forecasting. Based on the flow matching generative paradigm, UniTS constructs a deterministic evolution path from noise to targets under the guidance of task-specific conditions, achieving unified modeling of spatiotemporal representations for multi-level tasks. The UniTS architecture consists of a diffusion transformer with spatiotemporal blocks, where we design an Adaptive Condition Injector (ACor) to enhance the model's conditional perception of multimodal inputs, enabling high-quality controllable generation. Additionally, we design a Spatiotemporal-aware Modulator (STM) to improve the ability of spatiotemporal blocks to capture complex spatiotemporal dependencies. It substantially outperforms existing specialized models, particularly under challenging conditions such as severe cloud contamination, modality absence, and forecasting complex phenological variations.

==> related-works.tex <==
\subsection{Remote Sensing/Spectral Foundation Models}

FMs leverage SSL strategies to learn generalizable representations from large-scale unlabeled data, typically without being directly tailored for specific tasks \cite{chen2024internvl,xiong2024neural,lacoste2024geo}. For downstream tasks, supervised fine-tuning with labeled data is often required to better adapt FMs to specific application requirements. MAE \cite{he2022masked} is a commonly used SSL approach where parts of the input image are randomly masked, and the model is trained to reconstruct the masked regions, thus learning the underlying visual representations. Most RSFMs and SpectralFMs are adaptations and extensions of MAE for satellite remote sensing imagery. Scale-MAE \cite{reed2023scale} applies masking to the input image at predetermined scales for pre-training. By utilizing band-pass filters, it reconstructs low- and high-frequency images at different scales, thereby exploring robust multi-scale representations of remote sensing images. Cross-Scale MAE \cite{tang2024cross} introduces scale augmentation during pre-training phase and incorporates both contrastive and generative losses to enforce cross-scale consistency learning.

Further exploring the spectral modality, SatMAE introduced temporal encoding into satellite remote sensing imagery and assigned unique spectral positional encodings to MSI, thereby enhancing the model's ability to represent spectral information. Building upon SatMAE \cite{cong2022satmae}, SatMAE++ \cite{noman2024rethinking} further supports multi-scale pre-training and incorporates a convolution-based upsampling module to reconstruct finer image details at higher scales. SpectralGPT \cite{hong2024spectralgpt} adopts a progressive training strategy designed to accommodate input data with varying sizes, resolutions, temporal sequences, and regions. By designing three-dimensional tokens, it achieves deep coupling of spatial and spectral information. Furthermore, SpectralGPT employs multi-objective reconstruction tasks to effectively capture key information within spectral sequences. HyperSIGMA \cite{wang2024hypersigma} is specifically designed for HSI and pre-trained on the large-scale hyperspectral dataset HyperGlobal-450K. It introduces a novel sparse sampling attention mechanism and a spectral enhancement module designed to integrate both spatial and spectral features, providing a more comprehensive representation of the multi-dimensional properties of HSI. Li et al. proposed a hyperspectral FM without tuning (HyperFree) \cite{li2025hyperfree}, which can process arbitrary HSIs in a prompt or zero-shot manner in different tasks. The authors collected 41,946 hyperspectral images from AVIRIS airborne sensor and designed the Hyper-Seg data engine to build nearly 150,000 images and 15.44 million masks.

\subsection{Parameter-Efficient Fine-Tuning}
Given the powerful representation capabilities of FMs, fine-tuning FMs for downstream tasks has become a popular paradigm. However, while traditional full fine-tuning is effective, it requires substantial computational and memory resources, as well as a relatively large labeled dataset. This becomes particularly expensive for FMs with billions or even trillions of parameters. Recently, PEFT has emerged as a promising solution in natural language processing (NLP) \cite{houlsby2019parameter}, addressing these challenges by limiting the number of trainable parameters during the fine-tuning stage, while potentially achieving comparable or even better performance than full fine-tuning \cite{jia2022visual,fu2024dtl}. PEFT methods train only bias parameters and introduce additional trainable adapter modules, significantly reducing the number of learnable parameters \cite{han2024parameter}. This not only facilitates more efficient adaptation to new tasks but also preserves the knowledge already learned by the FMs. Dong et al. \cite{10735106} proposed Domain-Specific and General Knowledge Fusion (DSGF) by incorporating feature-matching scores for few-shot out-of-distribution detection under different fine-tuning paradigms. Wang et al. \cite{10770155} introduced the Hyper-Adaptive network (HAda) with weight-calibrated adapters to achieve specific information transfer between multiple views. Geospatial Domain Adaptation (GDA) \cite{scheibenreif2024parameter} incorporated a Scaled Low-Rank (SLR) adapter with a small number of parameters into pre-trained RSFMs, combining it with the SSL strategy of MAE to adapt to new data modalities. Automatic Labeling for Pre-training in Segmentation (ALPS) \cite{10949707} combined Segment Anything Model and K-means to predict pseudo labels of remote sensing images without prior annotation.
